Effidit: Your AI Writing Assistant

In this technical report, we introduce Effidit (Efficient and Intelligent Editing), a digital writing assistant that facilitates users to write higher-quality text more efficiently by using artificial intelligence (AI) technologies. Previous writing assistants typically provide the function of error checking (to detect and correct spelling and grammatical errors) and limited text-rewriting functionality. With the emergence of large-scale neural language models, some systems support automatically completing a sentence or a paragraph. In Effidit, we significantly expand the capacities of a writing assistant by providing functions in five categories: text completion, error checking, text polishing, keywords to sentences (K2S), and cloud input methods (cloud IME). In the text completion category, Effidit supports generation-based sentence completion, retrieval-based sentence completion, and phrase completion. In contrast, many other writing assistants so far only provide one or two of the three functions. For text polishing, we have three functions: (context-aware) phrase polishing, sentence paraphrasing, and sentence expansion, whereas many other writing assistants often support one or two functions in this category. The main contents of this report include major modules of Effidit, methods for implementing these modules, and evaluation results of some key methods.

==> Effidit new/Correction.tex <==
Given a piece of written text as the input, the task of grammatical error correction is to detect spelling and grammatical errors and give correction suggestions. 
Grammarly \cite{omelianchuk2020gector} achieves remarkable performance in handling grammatical errors in English text.
In this part, we describe our system for Chinese error correction.
Dominating error types in Chinese text include substitution, deletion, and insertion errors. 
We have a tail-to-tail model \cite{DBLP:conf/acl/Li020} to handle substitution errors and a tailored pretrained model \cite{zhouinsertbert2022} to handle deletion and insertion errors.


\subsubsection{Tail-to-Tail Non-Autoregressive Sequence Prediction}
Our first model is a non-autoregressive sequence-to-sequence model, abbreviated as \textbf{TtT}~\cite{DBLP:conf/acl/Li020}. We use the BERT encoder to produce the contextual vector representation for each token.
A Conditional Random Fields (CRF) \cite{DBLP:conf/icml/LaffertyMP01} layer is stacked on the up tail to model the dependencies among neighbouring tokens. The focal loss penalty strategy \cite{DBLP:journals/pami/LinGGHD20} is adopted to alleviate the class imbalance problem considering that most of the tokens in a sentence are not changed.


\subsubsection{Pretraining for Detecting Word Insertion and Deletion Errors}
Our second model is specifically designed to tackle insertion and deletion errors.
Recently, BERT and its model variations \cite{hong2019faspell,zhang-etal-2020-spelling,liu-etal-2021-plome} show promising results on handling grammatical errors related to word substitution. 
However, they do not perform well in handling word insertion and deletion errors.
The reason is that the learning objective of BERT assumes the existence of a word at each position, but this is incapable of determining whether no word exists at a position. 
Take word insertion as an example. If a word needs to be inserted between two words (i.e., $w_i$ and $w_{i+1}$), the standard BERT hardly detects anomalies because $w_i$ fits well into its preceding context and $w_{i+1}$ fits well into its following context. 

\begin{figure}[h]
	\centering
	\includegraphics[width=\textwidth]{figs/insertbert-case-study.pdf}
	\caption{Model outputs of InsertBERT for word deletion and insertion errors. Erroneous positions are highlighted in blue. }
	\label{fig:insertbert-case-study}
\end{figure}


We address the aforementioned problem with a tailored pretrained model named InsertBERT \cite{zhouinsertbert2022}.
The basic idea is to enable the model to determine whether a word exists at a particular position.
We achieve this by introducing a special token \texttt{[null]}, the prediction of which stands for the non-existence of a word.
In the training stage, we design pretraining tasks such that the model learns to predict \texttt{[null]} and real words jointly given the surrounding context. 
In the inference stage, the model readily detects whether a word should be inserted or deleted in the standard masked language modeling manner.
An additional advantage of the model is that it conducts detection and correction simultaneously because the top ranked real word can be directly used for error correction.

Figure \ref{fig:insertbert-case-study} shows the model outputs of InsertBERT for both deletion and insertion errors. We can see that InsertBERT is capable of handling both normal words (o1 and o3) and punctuations (o2 and o4). 

==> Effidit new/sentence_completion.tex <==
In this subsection we introduce the training and decoding methods of our generation-based sentence completion model.
One conventional approach is training a language model with a large corpus and decoding the most likely token as the next token.
However, since these models are usually trained with Maximum Likelihood Estimation (MLE), they may lead to a serious degeneration problem, i.e., the generated texts from the language model tend to be dull and contain undesirable repetitions at different levels (e.g., token-, phrase-, and sentence-level)~\cite{DBLP:journals/corr/abs-1902-00098}. Some examples of the degeneration problem are shown in Figure~\ref{fig:degeneration_example}, where we can find many repetitions.

\begin{figure}[h] 
  \centering    
  \setlength{\abovecaptionskip}{3pt}
  \includegraphics[width=0.8\textwidth]{figs/Figure_Completion_example.pdf}
  \caption{The degeneration problems in GPT-2}
  \label{fig:degeneration_example}
  \vspace{-1.5mm}
\end{figure}

We argue that this degeneration stems from the \textit{anisotropic} distribution of token representations, i.e., their representations reside in a narrow subset of the entire space~\cite{DBLP:conf/emnlp/Ethayarajh19,DBLP:conf/icml/DongCL21,su2021tacl}.
In Effidit, we implement \textit{SimCTG} (a \underline{\textbf{sim}}ple \underline{\textbf{c}}ontrastive framework for neural \underline{\textbf{t}}ext \underline{\textbf{g}}eneration)~\cite{su2022contrastive}, which encourages the model to learn discriminative and isotropic token representations.
A novel decoding strategy, \textit{contrastive search}, is also employed to complement SimCTG.
Key intuitions behind contrastive search are: (i) At each decoding step, the output should be selected from the set of most probable candidates predicted by the model to better maintain the semantic coherence between the generated text and the human-written prefix. (ii) The sparseness of the token similarity matrix of the generated text should be preserved to avoid degeneration.
For more details about SimCTG and its potential extensions, please refer to ~\cite{su2022contrastive, su2021tacl, su2022MAGIC}.


\subsubsection{Methodology}
In this section, we first present how to apply contrastive learning to calibrate the representation space of the language model. Then, we introduce the contrastive search decoding algorithm.

\paragraph{Contrastive Training}
\label{sec:contrastive_training}
Our goal is to encourage the language model to learn discriminative and isotropic token representations. To this end, a contrastive objective $\mathcal{L}_{\textup{CL}}$ is introduced into the training of the language model. Specifically, given a variable-length sequence $\boldsymbol{x}=\{x_1, ..., x_{|\boldsymbol{x}|}\}$, $\mathcal{L}_{\textup{CL}}$ is defined as 
\begin{equation}
    \label{eq:cl}
    \mathcal{L}_{\textup{CL}} = \frac{1}{|\boldsymbol{x}|\times(|\boldsymbol{x}| - 1)}\sum_{i=1}^{|\boldsymbol{x}|}\sum_{j=1,j\neq i}^{|\boldsymbol{x}|}\max\{0,\rho - s(h_{x_i}, h_{x_i}) + s(h_{x_i}, h_{x_j})\},
\end{equation}
where $\rho\in[-1,1]$ is a pre-defined margin and $h_{x_i}$ is the representation of token $x_i$ produced by the model. The similarity function $s$ computes the cosine similarity between token representations as
\begin{equation}
    \label{eq:cosine}
    s(h_{x_i}, h_{x_j}) = \frac{h_{x_i}^\top h_{x_j}}{\|h_{x_i}\|\cdot\|h_{x_j}\|}.
\end{equation}
Intuitively, by training with $\mathcal{L}_{\textup{CL}}$, the model learns to pull away the distances between representations of distinct tokens.\footnote{By definition, the cosine similarity $s(h_{x_i}, h_{x_i})$ of the identical token $x_i$ is $1.0$.} Therefore, a discriminative and isotropic model representation space can be obtained. The overall training objective $\mathcal{L}_{\textup{SimCTG}}$ is then defined as
\begin{equation}
    \label{eq:simctg}
    \mathcal{L}_{\textup{SimCTG}} = \mathcal{L}_{\textup{MLE}} + \mathcal{L}_{\textup{CL}},
\end{equation}
where the vanilla maximum likelihood estimation (MLE) objective $\mathcal{L}_{\textup{MLE}}$ is:
\begin{equation}
    \label{eq:mle}
    \mathcal{L}_{\textup{MLE}} = -\frac{1}{|\boldsymbol{x}|}\sum_{i=1}^{|\boldsymbol{x}|}\log p_{\theta}(x_i|\boldsymbol{x}_{<i}).
\end{equation} Note that, when the margin $\rho$ in $\mathcal{L}_{\textup{CL}}$ equals to $0$, the $\mathcal{L}_{\textup{SimCTG}}$ degenerates to the vanilla MLE objective $\mathcal{L}_{\textup{MLE}}$. 

\paragraph{Contrastive Search}
We employ a new decoding method called \textit{contrastive search}. At each decoding step, the key ideas of contrastive search are (i) the generated output should be selected from the set of most probable candidates predicted by the model; and (ii) the generated output should be discriminative enough with respect to the previous context. In this way, the generated text can better maintain semantic coherence with respect to the prefix while avoiding model degeneration.

Formally, given the context $\boldsymbol{x}_{<t}$, at time step $t$, the selection of the output $x_t$ follows
\begin{equation}
    \label{eq:score}
    x_t = \argmax_{v\in V^{(k)}}\bigg\{(1 - \alpha)\times \underbrace{p_{\theta}(v|\boldsymbol{x}_{<t})}_{\textup{model confidence}} -  \: \alpha \times \underbrace{(\max\{s(h_v, h_{x_j}):1\leq j \leq t-1\})}_{\textup{degeneration penalty}}\bigg\},
\end{equation}
where $V^{(k)}$ is the set of $k$ most-probable candidates predicted by the model $\theta$ and $k$ is typically set as 3$\sim$10. In Eq. \ref{eq:score}, the first term, \textit{model confidence}, is the probability of candidate $v$ predicted by the model. The second term, \textit{degeneration penalty}, measures how discriminative of candidate $v$ with respect to the previous context $\boldsymbol{x}_{<t}$ and $s$ is defined in Eq. \ref{eq:cosine}.
Specifically, it is defined as the maximum cosine similarity between the representation of $v$ and that of all tokens in $\boldsymbol{x}_{<t}$. Here, the candidate representation $h_v$ is computed by the model given the concatenation of $\boldsymbol{x}_{<t}$ and $v$.
Intuitively, a larger degeneration penalty of $v$ means it is more similar to the context, therefore more likely to lead to model degeneration.
The hyperparameter $\alpha\in[0,1]$ regulates the importance of the two components. When $\alpha=0$, contrastive search degenerates to the greedy search method.

\subsubsection{Experiments}
\label{sec:experiment}
We evaluate several approaches on the task of open-ended document generation.

\textbf{Model and Baselines.} SimCTG is architecture-agnostic and can be applied to any generation model.
In this work, we evaluate SimCTG on the representative GPT-2 model~\cite{radford2019language}.
Specifically, we fine-tune GPT-2 on the evaluation benchmark (detailed below) with the proposed objective $\mathcal{L}_{\textup{SimCTG}}$ (Eq. \ref{eq:simctg}) and generate the text continuation with different decoding methods.
Experiments are conducted using the base model (117M parameters) which consists of 12 Transformer layers~\cite{DBLP:conf/nips/VaswaniSPUJGKP17} with 12 attention heads.
SimCTG is compared with two strong baselines: (1) GPT-2 fine-tuned with the standard MLE objective (Eq. \ref{eq:mle}); and (2) GPT-2 fine-tuned with the unlikelihood objective ~\cite{DBLP:conf/iclr/WelleckKRDCW20}.\footnote{The unlikelihood baseline is implemented with the official code, which can be found here \url{https://github.com/facebookresearch/unlikelihood_training}.} Our implementation is based on the Huggingface library~\cite{DBLP:journals/corr/abs-1910-03771}.


\textbf{Evaluation Benchmark.} Experiments are conducted on the Wikitext-103 dataset ~\cite{DBLP:conf/iclr/MerityX0S17} which contains a large collection of Wikipedia articles with over 100 million words and 260 thousand unique tokens. Wikitext-103 is a document-level dataset and has been widely used for the evaluation of large-scale language modeling ~\cite{DBLP:conf/acl/DaiYYCLS19,DBLP:conf/iclr/KhandelwalLJZL20,DBLP:journals/tacl/YogatamadK21}.


\begin{table*}[h]
    \small
	\centering  
	\renewcommand{\arraystretch}{1.2}
	\setlength{\tabcolsep}{6pt}
	\scalebox{0.85}{
	\begin{tabular}{ccccc}
		%\hlinewd{0.75pt}
		\hline
        \textbf{Model}&Decoding Method&Coherence&Fluency&Informativeness\\
        \hline
        Agreement&-&0.51&0.64&0.70\\
        \hline
        \multirow{2}{*}{MLE}&nucleus&2.92&3.32&3.91\\
        &contrastive&2.78&2.29&2.56\\
        \hline
        \multirow{2}{*}{Unlikelihood}&nucleus&2.59&3.02&3.58\\
        &contrastive&2.76&2.90&3.35\\
        \hline
        \multirow{2}{*}{SimCTG}&nucleus&2.96&3.34&3.96\\
        &contrastive&3.25$^{\bigstar}$&3.57$^{\bigstar}$&3.96\\
        \hline
        \multirow{2}{*}{SimCTG-large}&nucleus&3.01&3.37&\textbf{3.98}\\
        &contrastive&\textbf{3.33}$^{\bigstar}$&\textbf{3.66}$^{\bigstar}$&\textbf{3.98}\\
        \hline
        Human&-&3.70&3.71&4.21\\
        \hline
		%\hlinewd{0.75pt}
	\end{tabular}}
    \caption{Human evaluation results. The results labeled with a star (${\bigstar}$) significantly outperform the corresponding nucleus sampling results (Sign test with p-value < 0.05).}
    	\vspace{-1.5mm}
	\label{tb:human_evaluation}
\end{table*}

\paragraph{Human Evaluation}
\label{sec:human_evaluation_detail}
Human evaluation is conducted with the help of graders proficient in English from a third-party annotation company. We randomly select 200 prefixes with a length of 32 from the test set of Wikitext-103. For each prefix, we use different models (MLE, Unlikelihood, and SimCTG) with two decoding methods (nucleus sampling and contrastive search) to generate text continuations with length of 128. The evaluation follows a 5-point Likert scale (1, 2, 3, 4, or 5) for each of the following features:
\begin{itemize}
    \item \textbf{Coherence}: Whether the generated text is semantically consistent with the prefix.
    \item \textbf{Fluency}: Whether the generated text is fluent and easy to understand.
    \item \textbf{Informativeness}: Whether the generated text is diverse and contains interesting content. 
\end{itemize}

Table \ref{tb:human_evaluation} presents the human evaluation results, with the first row showing strong inter-annotator agreements as measured by Fleiss$^\prime$ kappa coefficient~\cite{fleiss1971mns}. We observe that the results of SimCTG + contrastive search are significantly better than nucleus sampling with different models in terms of coherence and fluency (sign test with p-value $\textless$ 0.05). In addition, SimCTG-large + contrastive search achieves the best performance across the board and even performs comparably with human-written text on the fluency metric (sign test with p-value $\textgreater$ 0.4).
This reveals the clear generality of our approach to large size models. Future work could focus on extending it to models that contain over billions of parameters such as GPT-3~\cite{brown2020language}.

\begin{table*}[h]
    \small
	\centering  
	\renewcommand{\arraystretch}{1.2}
	\setlength{\tabcolsep}{6pt}
	\scalebox{0.75}{
	\begin{tabular}{ccccc}
		% \hlinewd{0.75pt}
		\hline
		\textbf{prefix}&\makecell[l]{Butt criticized Donald's controls in certain situations in the game, as well as the difficulty \\of some levels and puzzles. Buchanan also criticized the controls, calling}&div.&coh.&gen-ppl\\
		\hline
		
		beam&\makecell[l]{them " too easy " and " too difficult ". \textcolor{red}{He also criticized the game's graphics, stating that the game's}\\ \textcolor{red}{graphics were " too simplistic " and " too simplistic ".} He also criticized the game's graphics, stating\\ that the game's graphics were " too simplistic " and " too simplistic ". He also criticized the graphics,\\ stating that the game's graphics were " too simplistic " and " too simplistic ". He also criticized the\\ graphics, stating that the game's graphics were " too simplistic " and " too simplistic ". He also\\ criticized the graphics, stating that the game's graphics were" ...}&0.02&0.605&7.91\\
		\hline
		nucleus&\makecell[l]{them " offensively rudimentary ". After the game was released, Buchanan wrote a number of game\\ reviews about his review of the game, primarily summarizing what \textcolor{blue}{he thought the reviewers had}\\ \textcolor{blue}{enjoyed about it.} \textcolor{blue}{Buchanan was pleased with how consistently these reviews awarded the game.} \\For one, \textcolor{blue}{he praised the puzzles}, compared them to Nos. 1 and 2 and \textcolor{blue}{enjoyed the construction of the}\\ \textcolor{blue}{artificial intelligence in the game's forms}. \textcolor{blue}{He found no fault with the puzzles}, even in those situations\\ where they seemed repetitive. According to an Xbox Magazine review, " every time ...}&0.98&0.597&37.83\\
		\hline
		contrastive&\makecell[l]{them " unimpressive " and a " nightmare " of an experience to play with players unfamiliar with\\ Tetris. On the other hand, his opinion was shared by other reviewers, and some were critical of the\\ game's technical design for the Wii version of Tetris. In addition, Tintin's review included a quote\\ from Roger Ebert, who said that Tetris was better than the original game due to its simplicity and\\ ease of play. Ebert's comments were included in the game's DVD commentary, released on March\\ 22, 2010. It is unclear if any of the video commentary was taken from ...}&0.98&0.626&19.64\\
		%\hlinewd{0.75pt}
		\hline
	\end{tabular}}
    \caption{\textbf{Case study}: The beam search produces degeneration repetitions (highlighted in red) and the nucleus sampling produces text that has incoherent semantics with respect to the prefix (highlighted in blue). The ``div.'' and ``coh.'' stand for diversity and coherence metrics. (best viewed in color)}
    	%\vspace{-1.5mm}
	\label{tb:case_study}
\end{table*}



\paragraph{Case Study}
Table \ref{tb:case_study} shows some examples generated by SimCTG with different decoding methods given a specific prefix. We can see from the results that beam search produces undesirable sequence-level repetitions, resulting in low diversity and low generation perplexity.
On the other hand, in the prefix, the person ``Buchanan'' \textit{criticizes} the game.
However, the results from nucleus sampling contain contradicting statements, resulting in a low coherence score as well as a high generation perplexity. Lastly, for contrastive search, it generates text that is semantically consistent to the prefix with a proper perplexity while obtaining the same diversity as that of the nucleus sampling.



==> Effidit new/term_polishing.tex <==

Given a word or phrase in a sentence, the phrase polishing module suggests a list of word/phrase candidates that have similar semantic meaning to the input word/phrase and also fit the current context well.
Phrase polishing is fundamentally the context-aware semantic expansion task introduced in \cite{han2020case}, where a neural method was introduced to address the problem.
Since the neural method in that paper is quite time-consuming, a light-weight alternative approach is proposed in TexSmart \cite{zhang2020texsmart} to implement the semantic expansion of entities. We make an adaptation to this light-weight approach to support general words and phrases other than just entities.

Our phrase polishing approach includes an offline phase and an online phase.
In the offline phase, we build a similarity graph of words and phrases, where the similarity score is calculated by combining word embedding, distributional similarity, and pattern-based methods \cite{mikolov2013distributed, song2018directional, shi2010corpus}.
The graph is organized in a way that the top neighbors of a node can be retrieved efficiently.

In the online phase, the top neighbors of the input word/phrase are first retrieved from the graph as candidate results. Then a score is calculated for each candidate by considering two factors: the semantic similarity between the candidate and the input word/phrase, and the coherence between the candidate and the context of the input word/phrase in the sentence. Finally, the candidates are sorted by scores and the best scoring candidates are chosen as the phrase polishing results.

Now the core challenge is how to calculate the score of a candidate. We choose to compute the score as a linear combination of $S_1$ and $S_2$, where $S_1$ is the similarity between the candidate and the input word or phrase. Score $S_1$ can be obtained directly from the similarity graph, which has been built offline.

Score $S_2$ is adopted as an estimation of how well the candidate fits the context of the input word/phrase in the sentence.
Suppose $T$ is a candidate, and context $\mathbf{C}=\{c_1, c_2, \cdots, c_k\}$ is the set of words and phrases appearing in a window of the input word/phrase within the sentence. Score $S_2$ is calculated as:
\begin{equation}
  \textrm{$S_2$}(\mathbf{T}, \mathbf{C}) = \frac{1}{k}\sum_{x\in \mathbf{C}} \cos(v_x, w_T)
  \label{eq:s2}
\end{equation}
\noindent where $v_x$ denotes the input embedding of $x$, $w_y$ is the output word embedding of $T$ from a well-trained word embedding model, and $\cos$ is the cosine similarity function. 


==> Effidit new/text_expansion_and_rewriting.tex <==

\subsubsection{Sentence Paraphrasing}

Sentence paraphrasing is about rewriting a sentence with different words or syntactic structures while keeping the same semantics of the original sentence \cite{bhagat2013paraphrase,su2021keep}.
Rewriting provides users with new expressions and insights, which may inspire users to write more elegant text.

The biggest challenge in implementing text rewriting is how to acquire large-scale high-quality paraphrase pairs for training rewriting models.
In Effidit, we adopt three strategies to obtain the training data from various sources.

(1) Back translation\cite{federmann2019multilingual,mallinson2017paraphrasing}: We translate a sentence $S$ into sentence $T_1$ of another language and then translate it back to $T_2$ of the original language. Then the ($S$, $T_2$) pair is added to our training corpus of parallel text.

(2) Retrieval: Given a sentence, we retrieve the most similar sentences from a large-scale corpus using embedding-based retrieval technologies, where SimCSE \cite{gao2021simcse} is adopted as the text encoder and Faiss (Facebook AI Similarity Search) \cite{johnson2019billion} as the retrieval framework.

(3) Collecting existing text matching and paraphrase datasets \cite{liu2018lcqmc,chen2018bq}.

Some sentence pairs obtained from the above methods may not be good paraphrases.
So we delete the pairs with small lexical distances, by calculating their Levenshtein distance and WMD \cite{kusner2015word}.
We also remove the pairs with small semantic similarity, by training some text matching models, e.g., SimCSE \cite{gao2021simcse}.
We model text rewriting as a seq2seq learning task, and train a BART model \cite{lewis2019bart} from the sentence pairs after cleaning.
At inference time, the BART model takes the input sentence as input and outputs a list of paraphrase candidates.

\begin{table}[!hpb]
    \centering
    \small
    \begin{tabular}{c|l}

      Input   &  作文课上，刘老师带我们做了一个游戏。 \\ \\
      \multirow{2}{*}{Generated Output}   & 1. 本周的作文课上，和蔼的刘老师手把手带我们做了一个有趣的游戏。
      \\ & 2. 那天的作文课上，新来的刘老师兴致勃勃地带我们开心地做了一个益智游戏。
\\\hline
      Input   & 2020年7月4日，林丹发文宣布正式退出国家队。  \\ \\
      \multirow{2}{*}{Generated Output}   & 1. 2020年7月4日，中国名将林丹发文低调地宣布正式无限期退出羽毛球国家队。
      \\ & 2. 2020年7月4日，奥运冠军林丹在微博发文宣布从即日起正式退出曾经所在的国家队。

\\\hline
      Input   & 聂海胜谈中国航天员的未来：会刷新更多纪录。  \\ \\
      \multirow{2}{*}{Generated Output}   & 1. 宇航员聂海胜谈关于中国航天员的未来：太空探索会不断地刷新更多世界纪录。
      \\ & 2. 发言人聂海胜谈中国航天员的未来：载人航天会一次次的刷新更多史无前例的纪录。

    \end{tabular}
    \vspace{3mm}
    \caption{Examples of sentence expansion results generated by Effidit}
    \label{tab:expansion_example}
\end{table}

\subsubsection{Text Expansion}
Sentence expansion is about adding modifiers to an input sentence to make a longer one with rich information.
So far, only the Chinese version of text expansion is implemented in Effidit.
Some examples are shown in Table \ref{tab:expansion_example}.


Two approaches are employed in Effidit to generate expansion results: global expansion and local expansion.


\paragraph{Global Expansion}
In global expansion, a seq2seq model is trained from a large collection of (sentence, expanded-sentence) pairs.
Since these kinds of large-scale sentence pairs are not readily available, we choose to build pairs from sentences.
Given a sentence $S$, we first perform syntactic analysis (using TexSmart \cite{zhang2020texsmart}) to get its syntactic tree representation.
Then a skeleton $T$ of this sentence is obtained by randomly removing some modifiers from the syntactic tree. The $(T, S)$ pair is then treated as a (sentence, expanded-sentence) pair and added to our training data.
For example, given a sentence ``\textit{red is a powerful color that attracts more attention than probably any other color}''\footnote{Please note that, although we take an English sentence as an example here to illustrate our method, our current implementation is on Chinese text.}, if we extract ``\textit{red is a color}'' as one skeleton from the syntactic tree of the original sentence, the following pair can be obtained as one item in the training data:

\begin{center}
(``\textit{red is a color}'', ``\textit{red is a powerful color that attracts more attention than probably any other color}'')
\end{center}

A GPT-2 model \cite{gpt2} is then trained for text expansion based on our training data.
To fit the format of GPT-2, we concatenate the sentences in each pair with a special token ``[SEP]''. For example, if the pair is $(T, S)$, the input to GPT-2 during training is ``T [SEP] S [CLS]'', where ``[CLS]'' is an end indicator.
During inference, given sentence $T$, we use ``T [SEP]'' as the input to the GPT-2 model, and ask it to predict the expansion results.


\paragraph{Local Expansion}
In global expansion, the words or phrases to be enriched are decided by the seq2seq model itself and the decision principle is in a black box.
The goal of local expansion is to have more control about where to perform expansion.
The basic idea is to first choose one or a few places (mainly around a noun or verb) explicitly by a simple algorithm and then use a neural language model to predict some words or phrases that can be added to each place.
We call the two steps \textbf{space selection} and \textbf{modifier prediction}, respectively.
In our current implementation, space selection is based on the part-of-speech (POS) information of words and phrases, whereas modifier prediction is performed by the T5 pre-training model \cite{t5}.
Take the input sentence ``\textit{she saw flowers on the grass}'' as an example. Let's assume that two places are chosen in the space selection step: The first is before the word ``flower'', and the second is after the word ``grass''.
By inserting the ``[MASK]'' special token into the original sentence, we get,

\begin{center}
``\textit{she saw [MASK] flowers on the grass [MASK]}''
\end{center}

The above text is then sent to the T5 model for mask prediction.
Possible prediction results for the first mask might include ``\textit{colorful}'' , ``\textit{lovely}'', ``\textit{some beautiful}'', and the like. 
For the second mask, possible prediction results may include ``\textit{like natural rugs}'', ``\textit{in beautiful sunlight}'', etc.


==> Effidit new/text_infill.tex <==

We formulate the task of generation-based K2S as a text infilling problem, which is to generate missing spans of text.
Our system considers a general text infilling setting, where the incomplete sentence can contain an arbitrary number of blanks to be filled in, and each blank can involve an unknown number of tokens. Illustrated examples are provided in Table~\ref{tab:infill_example}.
\begin{table}[hpbp]
    \centering
    \small
    \begin{tabular}{c|l}
      Input (keywords)   &  春节,喜庆,团聚\\
      \multirow{2}{*}{Output (sentence)}   & \textbf{春节}是中华民族的传统节日，每年春节，家家户户都会举办一场\textbf{喜庆}的年俗活动，\\
      &来表达对新年的祝福和\textbf{团聚}
\\\hline
      Input (keywords) & rich, money, happy \\
      \multirow{2}{*}{Output (sentence)} & People who are \textbf{rich} and have \textbf{money} are more likely to be \textbf{happy} than those \\
      & who are poor.
\\\hline
      Input (keywords) & we observed, our model, promising results\\
      \multirow{2}{*}{Output (sentence)} & In this section, \textbf{we observed} that the architecture of \textbf{our model} neural network \\
      & is very \textbf{promising}.
    \end{tabular}
    \vspace{3mm}
    \caption{Example inputs and the generated infilled results}
    \label{tab:infill_example}
\end{table}


We implement our text infilling model by language modeling~\cite{Donahue2020EnablingLM}. An example for model training is constructed by masking random text segments of the raw data to generate an incomplete sentence as the input sequence with each mask segment replaced by a special token ``[blank]'', and its masked segments are concatenated as the output sequence with the special token ``[ans]'', as illustrated in Table~\ref{tab:data_example}. We then concatenate the input and output sequence with another special token (i.e. Input [seq] Output) and train an off-the-shelf language model. 

With a converged language model for inference, it takes the incomplete sentence as input and continues the input sentence until the number of generated special token ``[ans]'' equals to that of ``[blank]'' in the input sequence. We can obtain the complete sentence by filling the missing parts in the input sequence with the text spans between special tokens in the output sequence, sequentially.
\begin{table}[htbp]
    \centering
    \small
    \begin{tabular}{c|l}
      Data   & 今年春节到处喜庆洋洋，这是家家户户团聚的节日啊\\
      Input   & [blank]春节[blank]喜庆[blank]团聚[blank] \\
      Output & 今年[ans]到处[ans]洋洋，这是家家户户[ans]的节日啊[ans] \\ \hline
      Data & although they did not have a lot of money she says that she was never so happy. \\
      Input & [blank] money [blank] happy [blank]\\
      Output & although they did not have a lot of [ans] she says that she was never so [ans] . [ans]\\
    \end{tabular}
    \vspace{3mm}
    \caption{Constructed inputs and outputs for training language models}
    \label{tab:data_example}
\end{table}

\paragraph{Experiments}
Here, we train a GPT-2 with 12 Transformer layers from scratch with the 3 billion/3 billion  data constructed from about 1.5 billion /1.3 billion Chinese/English sentences. 
We randomly hold out 1000 test data for automatic and human evaluation.
Automatic evaluation metrics in our evaluation include Distinct-1/2~\cite{li2016diversity} (which calculates the ratio of unique 1/2 grams over all tokens in the test set) and Novelty (which calculates the ratio of added tokens over all tokens per test sample).
We also measure the Quality and Diversity by human annotation. The Quality contains two aspects: (1)~whether the result contains all given keywords and the order of keywords is consistent with the given one; (2)~language fluency. The Diversity measures how much degree the semantic of the infilled sentence is expanded from the incomplete sentence parts.
Five human annotators from a commercial annotating company evaluated the results of different methods using ratings from 1 to 5, where 5 is the best rating for Quality and Diversity. 

We compare our text infilling model by language modeling (LM) with other two  baselines: (i) Retrieval: Building an index for the training corpus and retrieving top sentences for the input keywords. BM25~\cite{robertson2009probabilistic} is adopted as the ranking function during the retrieval process. (ii) Masked language model by BERT~\cite{kenton2019bert}: We use the BERT model to predict a single token for each ``[blank]'' in the incomplete sentence. The results in Table~\ref{tab:text_infill_tab1} and Table~\ref{tab:text_infill_tab2} show that LM achieves the best performance on both sentence quality and diversity.

\begin{table}[htbp]
    \centering
    \begin{tabular}{lrrrrrr}
    \toprule
          & Dist-1 & Dist-2 & Novelty & Quality & Diversity \\\midrule
        LM  &0.76&0.92&5.42&3.57&4.32\\
        Retrieval & 0.93 &0.86&1.99&2.67&2.49\\
        BERT &0.95&0.89&2.10&2.13&2.36 \\
        \bottomrule
    \end{tabular}
    \vspace{3mm}
    \caption{Evaluation results for generation-based K2S on Chinese sentences}
    \label{tab:text_infill_tab1}
\end{table}

\begin{table}[htbp]
    \centering
    \begin{tabular}{lrrrrrr}
    \toprule
          & Dist-1 & Dist-2 & Novelty & Quality & Diversity \\\midrule
        LM  &0.87&0.94&5.81&4.28&4.02  \\
        Retrieval &0.97 &0.87  &2.10&2.40&1.76 \\
        BERT &0.91&0.88&1.86&1.82&2.15 \\
        \bottomrule
    \end{tabular}
    \vspace{3mm}
    \caption{Evaluation results for generation-based K2S on English sentences}
    \label{tab:text_infill_tab2}
\end{table}


==> Effidit new/ttt_pjli.tex <==


One model is tail-to-tail non-autoregressive sequence prediction, which abbreviated as \textbf{TtT}~\cite{DBLP:conf/acl/Li020}. Specifically, to directly convey the token information from the bottom tail to the up tail, a BERT based sequence encoder is introduced to conduct bidirectional representation learning.
For the input, we first obtain the representations by summing the word embeddings with the positional embeddings:
\begin{equation}
    \mathbf{H}^0_t = \mathbf{E}_{w_t}+\mathbf{E}_{p_t}
\end{equation}
where $0$ is the layer index and  $t$ is the state index. $\mathbf{E}_w$ and $\mathbf{E}_p$ are the embedding vectors for tokens and positions, respectively.
Then the obtained embedding vectors $\mathbf{H}^0$ are fed into several Transformer layers. Multi-head self-attention is used to conduct bidirectional representation learning:
\begin{equation}
\begin{split}
\mathrm{\bf H}^{1}_{t} &= \textsc{Ln}\left(\textsc{Ffn} (\mathrm{\bf H}^{1}_{t}) +\mathrm{\bf H}^1_t \right) \\
\mathrm{\bf H}^{1}_{t} &= \textsc{Ln}\left(\textsc{Slf-Att} (\mathrm{\bf Q}^{0}_{t}, \mathrm{\bf K}^{0}, \mathrm{\bf V}^{0}) +\mathrm{\bf H}^0_t \right) \\
\mathrm{\bf Q}^{0} &=  \mathrm{\bf H}^{0} \mathrm{\bf W}^{Q} \\
\mathrm{\bf K}^{0}, \mathrm{\bf V}^{0} &= \mathrm{\bf H}^{0}\mathrm{\bf W}^{K}, \mathrm{\bf H}^{0} \mathrm{\bf W}^{V}
\end{split}
\label{eql:formant_c1}
\end{equation}
where \textsc{Slf-Att}($\cdot$), \textsc{Ln}($\cdot$), and \textsc{Ffn}($\cdot$) represent self-attention mechanism, layer normalization, and feed-forward network respectively \cite{DBLP:conf/nips/VaswaniSPUJGKP17}. Note that our model is a non-autoregressive sequence prediction framework, thus we use all the sequence states $\mathrm{\bf K}^{0}$ and $\mathrm{\bf V}^{0}$ as the attention context. Then each node will absorb the context information bidirectionally. In order to conduct substitution, deletion, insertion, and local paraphrasing simultaneously, a Conditional Random Fields (CRF) \cite{DBLP:conf/icml/LaffertyMP01} layer is stacked on the up tail to conduct non-autoregressive sequence prediction by modeling the dependencies among neighbour tokens. Precisely, given the input sequence $X$, under the CRF framework, the likelihood of the target sequence $Y$ with length $T'$ is constructed as:
\begin{align}
\begin{split}
    P_\mathrm{crf}&({Y}|{X}) = \frac{1}{Z({X})}\exp\left(\sum_{t=1}^{T^{\prime}}s(y_t) + \sum_{t=2}^{T^{\prime}}t(y_{t-1},y_t)\right)
\end{split}
\end{align}
where $Z(X)$ is the normalizing factor and $s(y_t)$ represents the label score of $y$ at position $t$, which can be obtained from the predicted logit vector $\mathbf{s}_t \in \mathbb{R}^{|\mathcal{V}|}$, i.e., $\mathbf{s}_t(\mathcal{V}^{y_t})$, where $\mathcal{V}^{y_t}$ is the vocabulary index of token $y_t$. The value $t(y_{t-1},y_t)={\bf M}_{y_{t-1},y_t}$ denotes the transition score from token $y_{t-1}$ to $y_t$ where ${\bf M}\in\mathbb{R}^{|\mathcal{V}|\times |\mathcal{V}|}$ is the transition matrix, which is the core term to conduct dependency modeling. Usually, $\mathbf{M}$ can be learnt as neural network parameters during the end-to-end training procedure. However, $|\mathcal{V}|$ is typically very large especially in the text generation scenarios (more than $32k$), therefore it is infeasible to obtain $\mathbf{M}$ and $Z(X)$ efficiently in practice.
To overcome this obstacle, we employ two low-rank neural parameter metrics $\mathbf{E}_1$, $\mathbf{E}_2 \in \mathbb{R}^{|\mathcal{V}|\times d_m}$ to approximate the full-rank transition matrix $\mathbf{M}$ by:
\begin{equation}
\mathbf{M} = \mathbf{E}_1\mathbf{E}_2^\top
\end{equation}
where $d_m \ll |\mathcal{V}|$.
To compute the normalizing factor $Z(X)$, the original Viterbi algorithm need to search all paths. To improve the efficiency, here we only visit the truncated top-$k$ nodes at each time step approximately \cite{DBLP:conf/eacl/SuCWVBLC21}.
Low-rank decomposition and beamed Viterbi algorithm are introduced to accelerate the computations. Focal loss penalty strategy~\cite{DBLP:journals/pami/LinGGHD20} is adopted to alleviate the class imbalance problem considering that most of the tokens in a sentence are not changed.

Considering the characteristic of the directly bottom-to-up information conveying of the task CGEC, therefore, both tasks, direct prediction and CRF-based dependency modeling, can be incorporated jointly into a unified framework during the training stage. The reasons are that, intuitively, direct prediction will focus on the fine-grained predictions at each position, while CRF-layer will pay more attention to the high-level quality of the whole global sequence.
We employ Maximum Likelihood Estimation (MLE) to conduct parameter learning and treat negative log-likelihood (NLL) as the loss function. Thus, the optimization objective for direct prediction $\mathcal{L}_{\mathrm{dp}}$ is:
\begin{equation}
\begin{split}
\mathcal{L}_{\mathrm{dp}} = -\sum^{T'}_{t=1} \log P_{\mathrm{dp}}(\mathrm{y}_t|X)
\end{split}
\label{eq:nll_dp}
\end{equation}
And the loss function $\mathcal{L}_{\mathrm{crf}}$ for CRF-based dependency modeling is:
\begin{equation}
\begin{split}
\mathcal{L}_{\mathrm{crf}} = -\log P_\mathrm{crf}({Y}|{X})
\end{split}
\label{eq:nll_crf}
\end{equation}
Then the final optimization objective is:
\begin{equation}
\mathcal{L} = \mathcal{L}_{\mathrm{dp}} + \mathcal{L}_{\mathrm{crf}}
\end{equation}

One obvious but crucial phenomenon for CGEC is that most words in a sentence are correct and need not to be changed. Considering that maximum likelihood estimation is used as the parameter learning approach in those two tasks, then a simple copy strategy can lead to a sharp decline in terms of loss functions. Then, intuitively, the grammatical error tokens which need to be correctly fixed in practice, unfortunately, attract less attention during the training procedure. Actually, these tokens, instead, should be regarded as the focal points and contribute more to the optimization objectives. However, no previous works investigate this problem thoroughly on the task of CGEC.
To alleviate this issue, we introduce a useful trick, focal loss~\cite{DBLP:journals/pami/LinGGHD20} , into our loss functions for direct prediction and CRF:
\begin{align}
\begin{split}
\mathcal{L}_{\mathrm{dp}}^{\mathrm{fl}} &= -\sum^{T'}_{t=1} (1 - P_{\mathrm{dp}}(\mathrm{y}_t|X))^{\gamma} \log P_{\mathrm{dp}}(\mathrm{y}_t|X)\\
\mathcal{L}_{\mathrm{crf}}^{\mathrm{fl}} &= -(1 - P_\mathrm{crf}({Y}|{X}))^{\gamma}\log P_\mathrm{crf}({Y}|{X})
\end{split}
\end{align}
where $\gamma$ is a hyperparameter to control the penalty weight. It is obvious that $\mathcal{L}_{\mathrm{dp}}^{\mathrm{fl}}$ is penalized on the token level, while $\mathcal{L}_{\mathrm{crf}}^{\mathrm{fl}}$ is weighted on the sample level and will work in the  condition of batch-training. The final optimization objective with focal penalty strategy is:
\begin{equation}
\mathcal{L}^{\mathrm{fl}} = \mathcal{L}_{\mathrm{dp}}^{\mathrm{fl}} + \mathcal{L}_{\mathrm{crf}}^{\mathrm{fl}}
\end{equation}

\paragraph{Experiments} 
We conduct experimental evaluation and comparisons on the dataset of SIGHAN15~\cite{DBLP:conf/acl-sighan/TsengLCC15}, and we employ sentence-level \textbf{Accuracy}, \textbf{Precision}, \textbf{Recall}, and \textbf{F1-Measure} as the automatic metrics to evaluate the performance of all systems\footnote{\url{http://nlp.ee.ncu.edu.tw/resource/csc.html}}.
Table~\ref{tbl:results_sighan} depicts the main evaluation results of our proposed framework \textbf{TtT} as well as the comparison baseline methods. It should be emphasized that SoftMask-BERT is pre-trained on a 500M-size paired dataset. Our model TtT, as well as the baseline methods such as Transformer-s2s, GPT2-finetune, BERT-finetune, and Hybird are all trained on the 270k-size HybirdSet. Nevertheless, TtT obtains improvements on the tasks of error Detection and Correction compared to most of the strong baselines on F1 metric, which indicates the superiority of our proposed approach. 

\begin{table}[h]
\small
    \centering
    \resizebox{0.9\columnwidth}{!}{
    \begin{tabular}{l|cccc|cccc}
    \Xhline{3\arrayrulewidth}
     \multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{Detection}} & \multicolumn{4}{c}{\textbf{Correction}} \\ 
     \cline{2-9} & \textsc{Acc.} & \textsc{Prec.} & \textsc{Rec.} & \textsc{F1} & \textsc{Acc.} & \textsc{Prec.} & \textsc{Rec.} & \textsc{F1} \\
     \hline
    NTOU (\cite{DBLP:conf/acl-sighan/TsengLCC15}) & 42.2 & 42.2 & 41.8 & 42.0 & 39.0 & 38.1 & 35.2 & 36.6 \\
    NCTU-NTUT (\cite{DBLP:conf/acl-sighan/TsengLCC15}) & 60.1 & 71.7 & 33.6 & 45.7 & 56.4 & 66.3 & 26.1 & 37.5 \\
    HanSpeller++ (\cite{DBLP:conf/acl-sighan/ZhangXHZC15}) & 70.1 & 80.3 & 53.3 & 64.0 & 69.2 & 79.7 & 51.5 & 62.5 \\
    Hybird (\cite{DBLP:conf/emnlp/WangSLHZ18}) & - & 56.6 & 69.4 & 62.3 & - & - 
    & - & 57.1 \\
    FASPell (\cite{hong2019faspell}) & 74.2 & 67.6 & 60.0 & 63.5 & 73.7 & 66.6 & 59.1 & 62.6 \\
    Confusionset (\cite{DBLP:conf/acl/WangTZ19}) & - & 66.8 & 73.1 & 69.8 & - & 71.5 & 59.5 & 64.9 \\
    SoftMask-BERT (\cite{DBLP:conf/acl/ZhangHLL20}) & 80.9 & 73.7 & 73.2 & 73.5 & 77.4 & 66.7 & 66.2 & 66.4 \\
    \hline
    Transformer-s2s & 67.0 & 73.1 & 52.2 & 50.9 & 66.2 & 72.5 & 50.6 & 59.6\\
    GPT2-finetune  & 65.1 & 70.0 & 51.9 & 59.4 & 64.6 & 69.1 & 50.7 & 58.5\\
    BERT-finetune & 75.4 & 84.1 & 61.5 & 71.1 & 71.6 & 82.2 & 53.9 & 65.1\\
    \hline
    \textbf{TtT}  & 82.7 & 85.4 & 78.1 & 81.6 & 81.5 & 85.0 & 75.6 & 80.0 \\
    \Xhline{3\arrayrulewidth}
    \end{tabular}}
    \caption{Detection and Correction results evaluated on the SIGHAN2015 testset (1100 samples).} 
    \label{tbl:results_sighan}
\end{table}



==> ttt_pjli.tex <==


One model is tail-to-tail non-autoregressive sequence prediction, which abbreviated as \textbf{TtT}~\cite{DBLP:conf/acl/Li020}. Specifically, to directly convey the token information from the bottom tail to the up tail, a BERT based sequence encoder is introduced to conduct bidirectional representation learning.
For the input, we first obtain the representations by summing the word embeddings with the positional embeddings:
\begin{equation}
    \mathbf{H}^0_t = \mathbf{E}_{w_t}+\mathbf{E}_{p_t}
\end{equation}
where $0$ is the layer index and  $t$ is the state index. $\mathbf{E}_w$ and $\mathbf{E}_p$ are the embedding vectors for tokens and positions, respectively.
Then the obtained embedding vectors $\mathbf{H}^0$ are fed into several Transformer layers. Multi-head self-attention is used to conduct bidirectional representation learning:
\begin{equation}
\begin{split}
\mathrm{\bf H}^{1}_{t} &= \textsc{Ln}\left(\textsc{Ffn} (\mathrm{\bf H}^{1}_{t}) +\mathrm{\bf H}^1_t \right) \\
\mathrm{\bf H}^{1}_{t} &= \textsc{Ln}\left(\textsc{Slf-Att} (\mathrm{\bf Q}^{0}_{t}, \mathrm{\bf K}^{0}, \mathrm{\bf V}^{0}) +\mathrm{\bf H}^0_t \right) \\
\mathrm{\bf Q}^{0} &=  \mathrm{\bf H}^{0} \mathrm{\bf W}^{Q} \\
\mathrm{\bf K}^{0}, \mathrm{\bf V}^{0} &= \mathrm{\bf H}^{0}\mathrm{\bf W}^{K}, \mathrm{\bf H}^{0} \mathrm{\bf W}^{V}
\end{split}
\label{eql:formant_c1}
\end{equation}
where \textsc{Slf-Att}($\cdot$), \textsc{Ln}($\cdot$), and \textsc{Ffn}($\cdot$) represent self-attention mechanism, layer normalization, and feed-forward network respectively \cite{DBLP:conf/nips/VaswaniSPUJGKP17}. Note that our model is a non-autoregressive sequence prediction framework, thus we use all the sequence states $\mathrm{\bf K}^{0}$ and $\mathrm{\bf V}^{0}$ as the attention context. Then each node will absorb the context information bidirectionally. In order to conduct substitution, deletion, insertion, and local paraphrasing simultaneously, a Conditional Random Fields (CRF) \cite{DBLP:conf/icml/LaffertyMP01} layer is stacked on the up tail to conduct non-autoregressive sequence prediction by modeling the dependencies among neighbour tokens. Precisely, given the input sequence $X$, under the CRF framework, the likelihood of the target sequence $Y$ with length $T'$ is constructed as:
\begin{align}
\begin{split}
    P_\mathrm{crf}&({Y}|{X}) = \frac{1}{Z({X})}\exp\left(\sum_{t=1}^{T^{\prime}}s(y_t) + \sum_{t=2}^{T^{\prime}}t(y_{t-1},y_t)\right)
\end{split}
\end{align}
where $Z(X)$ is the normalizing factor and $s(y_t)$ represents the label score of $y$ at position $t$, which can be obtained from the predicted logit vector $\mathbf{s}_t \in \mathbb{R}^{|\mathcal{V}|}$, i.e., $\mathbf{s}_t(\mathcal{V}^{y_t})$, where $\mathcal{V}^{y_t}$ is the vocabulary index of token $y_t$. The value $t(y_{t-1},y_t)={\bf M}_{y_{t-1},y_t}$ denotes the transition score from token $y_{t-1}$ to $y_t$ where ${\bf M}\in\mathbb{R}^{|\mathcal{V}|\times |\mathcal{V}|}$ is the transition matrix, which is the core term to conduct dependency modeling. Usually, $\mathbf{M}$ can be learnt as neural network parameters during the end-to-end training procedure. However, $|\mathcal{V}|$ is typically very large especially in the text generation scenarios (more than $32k$), therefore it is infeasible to obtain $\mathbf{M}$ and $Z(X)$ efficiently in practice.
To overcome this obstacle, we employ two low-rank neural parameter metrics $\mathbf{E}_1$, $\mathbf{E}_2 \in \mathbb{R}^{|\mathcal{V}|\times d_m}$ to approximate the full-rank transition matrix $\mathbf{M}$ by:
\begin{equation}
\mathbf{M} = \mathbf{E}_1\mathbf{E}_2^\top
\end{equation}
where $d_m \ll |\mathcal{V}|$.
To compute the normalizing factor $Z(X)$, the original Viterbi algorithm need to search all paths. To improve the efficiency, here we only visit the truncated top-$k$ nodes at each time step approximately \cite{DBLP:conf/eacl/SuCWVBLC21}.
Low-rank decomposition and beamed Viterbi algorithm are introduced to accelerate the computations. Focal loss penalty strategy~\cite{DBLP:journals/pami/LinGGHD20} is adopted to alleviate the class imbalance problem considering that most of the tokens in a sentence are not changed.

Considering the characteristic of the directly bottom-to-up information conveying of the task CGEC, therefore, both tasks, direct prediction and CRF-based dependency modeling, can be incorporated jointly into a unified framework during the training stage. The reasons are that, intuitively, direct prediction will focus on the fine-grained predictions at each position, while CRF-layer will pay more attention to the high-level quality of the whole global sequence.
We employ Maximum Likelihood Estimation (MLE) to conduct parameter learning and treat negative log-likelihood (NLL) as the loss function. Thus, the optimization objective for direct prediction $\mathcal{L}_{\mathrm{dp}}$ is:
\begin{equation}
\begin{split}
\mathcal{L}_{\mathrm{dp}} = -\sum^{T'}_{t=1} \log P_{\mathrm{dp}}(\mathrm{y}_t|X)
\end{split}
\label{eq:nll_dp}
\end{equation}
And the loss function $\mathcal{L}_{\mathrm{crf}}$ for CRF-based dependency modeling is:
\begin{equation}
\begin{split}
\mathcal{L}_{\mathrm{crf}} = -\log P_\mathrm{crf}({Y}|{X})
\end{split}
\label{eq:nll_crf}
\end{equation}
Then the final optimization objective is:
\begin{equation}
\mathcal{L} = \mathcal{L}_{\mathrm{dp}} + \mathcal{L}_{\mathrm{crf}}
\end{equation}

One obvious but crucial phenomenon for CGEC is that most words in a sentence are correct and need not to be changed. Considering that maximum likelihood estimation is used as the parameter learning approach in those two tasks, then a simple copy strategy can lead to a sharp decline in terms of loss functions. Then, intuitively, the grammatical error tokens which need to be correctly fixed in practice, unfortunately, attract less attention during the training procedure. Actually, these tokens, instead, should be regarded as the focal points and contribute more to the optimization objectives. However, no previous works investigate this problem thoroughly on the task of CGEC.
To alleviate this issue, we introduce a useful trick, focal loss~\cite{DBLP:journals/pami/LinGGHD20} , into our loss functions for direct prediction and CRF:
\begin{align}
\begin{split}
\mathcal{L}_{\mathrm{dp}}^{\mathrm{fl}} &= -\sum^{T'}_{t=1} (1 - P_{\mathrm{dp}}(\mathrm{y}_t|X))^{\gamma} \log P_{\mathrm{dp}}(\mathrm{y}_t|X)\\
\mathcal{L}_{\mathrm{crf}}^{\mathrm{fl}} &= -(1 - P_\mathrm{crf}({Y}|{X}))^{\gamma}\log P_\mathrm{crf}({Y}|{X})
\end{split}
\end{align}
where $\gamma$ is a hyperparameter to control the penalty weight. It is obvious that $\mathcal{L}_{\mathrm{dp}}^{\mathrm{fl}}$ is penalized on the token level, while $\mathcal{L}_{\mathrm{crf}}^{\mathrm{fl}}$ is weighted on the sample level and will work in the  condition of batch-training. The final optimization objective with focal penalty strategy is:
\begin{equation}
\mathcal{L}^{\mathrm{fl}} = \mathcal{L}_{\mathrm{dp}}^{\mathrm{fl}} + \mathcal{L}_{\mathrm{crf}}^{\mathrm{fl}}
\end{equation}

\paragraph{Experiments} 
We conduct experimental evaluation and comparisons on the dataset of SIGHAN15~\cite{DBLP:conf/acl-sighan/TsengLCC15}, and we employ sentence-level \textbf{Accuracy}, \textbf{Precision}, \textbf{Recall}, and \textbf{F1-Measure} as the automatic metrics to evaluate the performance of all systems\footnote{\url{http://nlp.ee.ncu.edu.tw/resource/csc.html}}.
Table~\ref{tbl:results_sighan} depicts the main evaluation results of our proposed framework \textbf{TtT} as well as the comparison baseline methods. It should be emphasized that SoftMask-BERT is pre-trained on a 500M-size paired dataset. Our model TtT, as well as the baseline methods such as Transformer-s2s, GPT2-finetune, BERT-finetune, and Hybird are all trained on the 270k-size HybirdSet. Nevertheless, TtT obtains improvements on the tasks of error Detection and Correction compared to most of the strong baselines on F1 metric, which indicates the superiority of our proposed approach. 

\begin{table}[h]
\small
    \centering
    \resizebox{0.9\columnwidth}{!}{
    \begin{tabular}{l|cccc|cccc}
    \Xhline{3\arrayrulewidth}
     \multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{Detection}} & \multicolumn{4}{c}{\textbf{Correction}} \\ 
     \cline{2-9} & \textsc{Acc.} & \textsc{Prec.} & \textsc{Rec.} & \textsc{F1} & \textsc{Acc.} & \textsc{Prec.} & \textsc{Rec.} & \textsc{F1} \\
     \hline
    NTOU (\cite{DBLP:conf/acl-sighan/TsengLCC15}) & 42.2 & 42.2 & 41.8 & 42.0 & 39.0 & 38.1 & 35.2 & 36.6 \\
    NCTU-NTUT (\cite{DBLP:conf/acl-sighan/TsengLCC15}) & 60.1 & 71.7 & 33.6 & 45.7 & 56.4 & 66.3 & 26.1 & 37.5 \\
    HanSpeller++ (\cite{DBLP:conf/acl-sighan/ZhangXHZC15}) & 70.1 & 80.3 & 53.3 & 64.0 & 69.2 & 79.7 & 51.5 & 62.5 \\
    Hybird (\cite{DBLP:conf/emnlp/WangSLHZ18}) & - & 56.6 & 69.4 & 62.3 & - & - 
    & - & 57.1 \\
    FASPell (\cite{hong2019faspell}) & 74.2 & 67.6 & 60.0 & 63.5 & 73.7 & 66.6 & 59.1 & 62.6 \\
    Confusionset (\cite{DBLP:conf/acl/WangTZ19}) & - & 66.8 & 73.1 & 69.8 & - & 71.5 & 59.5 & 64.9 \\
    SoftMask-BERT (\cite{DBLP:conf/acl/ZhangHLL20}) & 80.9 & 73.7 & 73.2 & 73.5 & 77.4 & 66.7 & 66.2 & 66.4 \\
    \hline
    Transformer-s2s & 67.0 & 73.1 & 52.2 & 50.9 & 66.2 & 72.5 & 50.6 & 59.6\\
    GPT2-finetune  & 65.1 & 70.0 & 51.9 & 59.4 & 64.6 & 69.1 & 50.7 & 58.5\\
    BERT-finetune & 75.4 & 84.1 & 61.5 & 71.1 & 71.6 & 82.2 & 53.9 & 65.1\\
    \hline
    \textbf{TtT}  & 82.7 & 85.4 & 78.1 & 81.6 & 81.5 & 85.0 & 75.6 & 80.0 \\
    \Xhline{3\arrayrulewidth}
    \end{tabular}}
    \caption{Detection and Correction results evaluated on the SIGHAN2015 testset (1100 samples).} 
    \label{tbl:results_sighan}
\end{table}


